Block Diffusion: Interpolating Between Autoregressive and Diffusion Language Models

Diffusion language models offer unique benefits over autoregressive models due to their potential for parallelized generation and controllability, yet they lag in likelihood modeling and are limited to fixed-length generation. In this work, we introduce a class of block diffusion language models that interpolate between discrete denoising diffusion and autoregressive models. Block diffusion overcomes key limitations of both approaches by supporting flexible-length generation and improving inference efficiency with KV caching and parallel token sampling. We propose a recipe for building effective block diffusion models that includes an efficient training algorithm, estimators of gradient variance, and data-driven noise schedules to minimize the variance. Block diffusion sets a new state-of-the-art performance among diffusion models on language modeling benchmarks and enables generation of arbitrary-length sequences. We provide the code, along with the model weights and blog post on the project page: https://m-arriola.com/bd3lms

==> algs/inference_alg.tex <==
\begin{algorithm}
\caption{SAR Inference}
\begin{algorithmic}[1]
\State \textbf{Input:} $p_{limit}$, $T$ diffusion steps, $L$ context length, $L'$ block length, $R$ layers
\State \textbf{Output:} $\tilde{\x}^0$

\State $\tilde{\x}^T \sim p_{limit}$
\Comment{Initialize noisy sample}

\State $\bar{K}, \bar{V} \gets \emptyset$
\Comment{kv cache}

\For{$i = 1$ to $\frac{L}{L'}$}
    \For{$t = T$ to $1$}
        \State $h^1 \gets \text{Linear}(\x^t_{(i-1)L':iL'}) + \text{PE}(\x^t)_{(i-1)L':iL'}$
        \Comment{vocab embed}
        
        \For{$r = 1$ to $R$}
            \State $Q^r, K^r, V^r \gets \text{Linear}(h^r_{(i-1)L':iL'})$
            \Comment{query block $i$}
            
            \State $K^r \gets \bar{K}^r_{0:(i-1)L'} \oplus K^r_{(i-1)L':iL'}$
            \Comment{use kv cache}
            
            \State $V^r \gets \bar{V}^r_{0:(i-1)L'} \oplus V^r_{(i-1)L':iL'}$
            
            \State $h^r_{(i-1)L':iL'} \gets \text{CrossAttn}(Q^r_{(i-1)L':iL'}, K^r_{0:iL'}, V^r_{0:iL'})$
            
            \State $h^r_{(i-1)L':iL'} \gets \text{Norm}(\text{MLP}(h^r_{(i-1)L':iL'}))$
            
            \State $h^{r+1} \gets h^{r+1} \oplus h^r_{(i-1)L':iL'}$
        \EndFor
        
        \State $\x^{t-1}_{iL':(i+1)L'} \sim h_R$
        \Comment{denoised sample}
    \EndFor
    
    \Comment{Update kv cache after sampling block $i$}
    \State $\bar{K}_{0:iL'} \gets \bar{K}_{0:(i-1)L'} \oplus K_{(i-1)L':iL'}$
    \State $\bar{V}_{0:iL'} \gets \bar{V}_{0:(i-1)L'} \oplus V_{(i-1)L':iL'}$
\EndFor

\State \Return $\x^0$
\end{algorithmic}
\end{algorithm}

==> algs/train_alg.tex <==
\begin{algorithm}
\caption{SAR Training}
\begin{algorithmic}[1]
\State \textbf{Input:} $p_{data}$, $L$ context length, $L'$ block length, $R$ layers
\While{not converged}
    \State $\x^0 \sim p_{data}$
    \Comment{Prefilling: block-causal masking}
    
    \State $h^1 \gets  \text{Linear}(\x^0) + \text{PE}(\x^0)$
    \Comment{vocab embed}
    
    \State $\bar{K}, \bar{V} \gets \emptyset$
    \Comment{kv cache}
    
    \State $M \gets \text{CreateMask}(L, L')$
    \Comment{block-causal mask}
    
    \For{$r = 1$ to $R$}
        \State $Q^r, K^r, V^r \gets \text{Linear}(h^r)$
        \State $\bar{K}^{r} \gets K^r$
        \Comment{update cache}
        
        \State $\bar{V}^{r} \gets \bar{V}^{r}$
        
        \State $h^{r+1} \gets \text{Attn}(Q^r, K^r, V^r, M)$
        \State $h^{r+1} \gets \text{Norm}(\text{MLP}(h^{r+1}))$
    \EndFor
    
    \Comment{Denoising: block-level random masking}
    
    \For{$i = 1$ to $\frac{L}{L'}$}
        \State $t \sim \mathcal{U}([0, 1])$
        
        \State $\x^t_{(i-1)L':iL'} \gets \text{noise}(\x^0_{(i-1)L':iL'}, t)$
        
        \State $h^1 \gets \text{Linear}(\x^t_{(i-1)L':iL'}) + \text{PE}(\x^t)_{(i-1)L':iL'}$
        \Comment{vocab embed}
        
        \For{$r = 1$ to $R$}
            \State $Q^r, K^r, V^r \gets \text{Linear}(h^r_{(i-1)L':iL'})$
            \Comment{block-level attention}
            
            \State $K^r \gets \bar{K}^r_{0:(i-1)L'} \oplus K^r$
            \Comment{use kv from prefilling}
            
            \State $V^r \gets \bar{V}^r_{0:(i-1)L'} \oplus V^r$
            
            \Comment{cross attention}
            
            \State $h^{r+1}_{(i-1)L':iL'} \gets \text{Attn}(Q^r_{(i-1)L':iL'}, K^r_{0:iL'}, V^r_{0:iL'})$
            
            \State $h^{r+1}_{(i-1)L':iL'} \gets \text{Norm}(\text{MLP}(h^{r+1}_{(i-1)L':iL'}))$
        \EndFor
    \EndFor
    
    \State $\x^0 \gets \text{Linear}(h^R)$
    
    \State Take gradient step on $\nabla \mathbb{E}_{t \sim (0, 1], q} \left[ \frac{\alpha_t'}{1-\alpha_t} \log \langle  \x_\theta(\z_t^b), \x_^b \rangle \right]$
    \Comment{SAR likelihood}
    
\EndWhile
\end{algorithmic}
\end{algorithm}

